BWLer: Barycentric Weight Layer Elucidates a Precision-Conditioning Tradeoff for PINNs

Physics-informed neural networks (PINNs) offer a flexible way to solve partial differential equations (PDEs) with machine learning, yet they still fall well short of the machine-precision accuracy many scientific tasks demand. In this work, we investigate whether the precision ceiling comes from the ill-conditioning of the PDEs or from the typical multi-layer perceptron (MLP) architecture. We introduce the Barycentric Weight Layer (BWLer), which models the PDE solution through barycentric polynomial interpolation. A BWLer can be added on top of an existing MLP (a BWLer-hat) or replace it completely (explicit BWLer), cleanly separating how we represent the solution from how we take derivatives for the PDE loss. Using BWLer, we identify fundamental precision limitations within the MLP: on a simple 1-D interpolation task, even MLPs with O(1e5) parameters stall around 1e-8 RMSE -- about eight orders above float64 machine precision -- before any PDE terms are added. In PDE learning, adding a BWLer lifts this ceiling and exposes a tradeoff between achievable accuracy and the conditioning of the PDE loss. For linear PDEs we fully characterize this tradeoff with an explicit error decomposition and navigate it during training with spectral derivatives and preconditioning. Across five benchmark PDEs, adding a BWLer on top of an MLP improves RMSE by up to 30x for convection, 10x for reaction, and 1800x for wave equations while remaining compatible with first-order optimizers. Replacing the MLP entirely lets an explicit BWLer reach near-machine-precision on convection, reaction, and wave problems (up to 10 billion times better than prior results) and match the performance of standard PINNs on stiff Burgers' and irregular-geometry Poisson problems. Together, these findings point to a practical path for combining the flexibility of PINNs with the precision of classical spectral solvers.

==> sections/fig1.tex <==
\centering
\begin{tikzpicture}[scale=\figonescale, every node/.style={scale=\figonescale}]

  \begin{axis}[
      view        = {40}{25},
      hide axis,
      domain      = -\PlaneSize/2:\PlaneSize/2,
      y domain    = -\PlaneSize/2:\PlaneSize/2,
      samples     = 15, samples y = 15,
      mesh/rows   = \GridN, mesh/cols = \GridN,
      shader      = flat,
      z buffer    = sort,
    ]

    % grey plane
    \addplot3[surf, color=PlaneCol, forget plot]{\PlaneZ};

    % plane lattice
    \DrawPlaneGrid

    % green samples + MLP arrows/boxes
    \DrawRandomSamplesMLP

    % blue surface
    \addplot3[surf, shader=flat, colormap name=solidSurf,
      opacity=0.35, forget plot]{\SurfExpr{x}{y}};
    % … inside your \begin{axis}[…] … \end{axis} …
    % 1) Place a node for your annotation text at any TikZ coordinate 
    %    (or axis‐relative coordinate) you choose:
    % \node[black, font=\LARGE, anchor=west] (ann1) at (axis cs:1.4, 1.5, 0.5)
    % {MLP};

    % 2) Draw a thin black arrow from that node back to the feature:
    % \draw[->, thin, black] (ann1) -- (axis cs:1.25, 0.8, 0.75);

  \end{axis}
  \node[draw=black, thick, fill=white, rounded corners=1pt,
    font=\bfseries\Large, anchor=south]
  at ($(current bounding box.north) + (0,0.4)$) {PINN};

\end{tikzpicture}
\centering
\begin{tikzpicture}[scale=\figonescale, every node/.style={scale=\figonescale}]
  \begin{axis}[
      view        = {40}{25},
      hide axis,
      domain      = -\PlaneSize/2:\PlaneSize/2,
      y domain    = -\PlaneSize/2:\PlaneSize/2,
      samples     = 15, samples y = 15,
      mesh/rows   = \GridN, mesh/cols = \GridN,
      shader      = flat,
      z buffer    = sort,
    ]

    % grey plane
    \addplot3[surf, color=PlaneCol, forget plot]{\PlaneZ};

    % plane lattice
    \DrawPlaneGrid

    \DrawRandomSamplesBWLER

    % --- vertical stalks (no dots) ---
    \DrawStalksHatted

    % blue surface
    \addplot3[surf, shader=flat, colormap name=solidSurf,
      opacity=0.35, forget plot]{\SurfExpr{x}{y}};

  \end{axis}
  \node[draw=black, thick, fill=white, rounded corners=1pt,
    font=\bfseries\Large, anchor=south]
  at ($(current bounding box.north) + (0,0.4)$) {\methodname-hatted PINN};

\end{tikzpicture}
\centering
\begin{tikzpicture}[scale=\figonescale, every node/.style={scale=\figonescale}]

  \begin{axis}[
      view        = {40}{25},
      hide axis,
      domain      = -\PlaneSize/2:\PlaneSize/2,
      y domain    = -\PlaneSize/2:\PlaneSize/2,
      % -- surface resolution vs mesh spacing --
      samples     = 15,   % controls smoothness of fill
      samples y   = 15,
      mesh/rows   = \GridN,   % controls how many visible grid lines
      mesh/cols   = \GridN,
      % mesh line style={surf mesh line},
      shader      = flat,
      z buffer    = sort,
      clip = false
    ]

    % --- gray plane ---
    \addplot3[surf, color=PlaneCol, forget plot]{\PlaneZ};

    % --- plane lattice ---
    \DrawPlaneGrid

    % --- blue surface with built‑in coarse mesh ---
    \addplot3[surf, shader=flat, colormap name=solidSurf,
      color=SurfCol, opacity=0.35, forget plot]{\SurfExpr{x}{y}};

    % --- vertical stalks (no dots) ---
    \DrawStalksUnhatted

    \DrawRandomSamplesBWLER

    % \node[black, font=\LARGE, anchor=west] (ann1) at (axis cs:-2.5, -2.5, -0.5)
    % {Barycentric Interpolation};

    % 2) Draw a thin black arrow from that node back to the feature:
    % \draw[->, thin, black] (ann1) -- (axis cs:0.2, -1.2, 0);

  \end{axis}
  \node[draw=black, thick, fill=white, rounded corners=1pt,
    font=\bfseries\Large, anchor=south]
  at ($(current bounding box.north) + (0,0.4)$) {\methodname};
\end{tikzpicture}


==> sections/scratch.tex <==
\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

% \subsection{Theorems and such}
% The preferred way is to number definitions, propositions, lemmas, etc. consecutively, within sections, as shown below.
% \begin{definition}
% \label{def:inj}
% A function $f:X \to Y$ is injective if for any $x,y\in X$ different, $f(x)\ne f(y)$.
% \end{definition}
% Using \cref{def:inj} we immediate get the following result:
% \begin{proposition}
% If $f$ is injective mapping a set $X$ to another set $Y$, 
% the cardinality of $Y$ is at least as large as that of $X$
% \end{proposition}
% \begin{proof} 
% Left as an exercise to the reader. 
% \end{proof}
% \cref{lem:usefullemma} stated next will prove to be useful.
% \begin{lemma}
% \label{lem:usefullemma}
% For any $f:X \to Y$ and $g:Y\to Z$ injective functions, $f \circ g$ is injective.
% \end{lemma}
% \begin{theorem}
% \label{thm:bigtheorem}
% If $f:X\to Y$ is bijective, the cardinality of $X$ and $Y$ are the same.
% \end{theorem}
% An easy corollary of \cref{thm:bigtheorem} is the following:
% \begin{corollary}
% If $f:X\to Y$ is bijective, 
% the cardinality of $X$ is at least as large as that of $Y$.
% \end{corollary}
% \begin{assumption}
% The set $X$ is finite.
% \label{ass:xfinite}
% \end{assumption}
% \begin{remark}
% According to some, it is only the finite case (cf. \cref{ass:xfinite}) that is interesting.
% \end{remark}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
\caption{Historical locations and number of accepted papers for International
Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
produced, the number of accepted papers for ICML 2008 was unknown and instead
estimated.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

% \begin{algorithm}[tb]
%    \caption{Bubble Sort}
%    \label{alg:example}
% \begin{algorithmic}
%    \STATE {\bfseries Input:} data $x_i$, size $m$
%    \REPEAT
%    \STATE Initialize $noChange = true$.
%    \FOR{$i=1$ {\bfseries to} $m-1$}
%    \IF{$x_i > x_{i+1}$}
%    \STATE Swap $x_i$ and $x_{i+1}$
%    \STATE $noChange = false$
%    \ENDIF
%    \ENDFOR
%    \UNTIL{$noChange$ is $true$}
% \end{algorithmic}
% \end{algorithm}

\footnote{Footnotes should be complete sentences.}
